Aggregate Cyber-Risk Management in the IoT Age: Cautionary Statistics for (Re)Insurers and Likes

In this paper, we provide (i) a rigorous general theory to elicit conditions on (tail-dependent) heavy-tailed cyber-risk distributions under which a risk management firm might find it (non)sustainable to provide aggregate cyber-risk coverage services for smart societies, and (ii)a real-data driven numerical study to validate claims made in theory assuming boundedly rational cyber-risk managers, alongside providing ideas to boost markets that aggregate dependent cyber-risks with heavy-tails.To the best of our knowledge, this is the only complete general theory till date on the feasibility of aggregate cyber-risk management.

==> Intro.tex <==
\section{Introduction}
Global commerce is undergoing a profound digital transformation. As it becomes increasingly electronic and IoT-driven, critical exposures in this sector are getting highly data-driven. As a result, the majority of modern business and economic risks are becoming increasingly cyber in nature. More importantly, such cyber-risks are often correlated and networked (thus inter-dependent), and accumulate in a variety of ways, thereby affecting many lines of business.  For instance, firms in diverse sectors such as automobiles, electronics, energy, finance, aerospace, etc., and their business and vendor relationships are characterized by systemic network linkages through major software providers (e.g., Oracle for DBMS support).  Consequently a cyber-attack exploiting a software vulnerability can have a catastrophic cascading service disruption effect that could amount to losses in billions of dollars across various service sectors. Recent examples of such cyber-attacks include the \emph{Mirai} DDoS (2016), \emph{NotPetya} ransomware (2017), and \emph{WannaCry} ransomware (2017) attacks, which wrecked havoc among firms in various industries across the globe, resulting in huge financial losses due to service interruption (see \cite{coburn2018solving} for more examples). 

%\subsection{Research Motivation}
%In the wake of major targeted corporate and critical infrastructure cyber-attacks (e.g., attacks on Sony, Target, Ukraine power grid) in the past half decade, risk mitigation has become a top board-level concern across many organizations worldwide. 
This reality has fueled significant rise in spending, in not only risk mitigation in the form of advanced security products, but also risk transfer/management in the form of cyber-insurance, 
%As a result, transfer based risk management products like cyber-insurance, 
a rapidly growing market\footnote{Recently, the \emph{Wired} magazine (2019) projected a huge US\$5500 billion cyber-insurance market by 2030 \cite{betterley2015cyber}.}. 
%, Advisen annual report 2016) is a major go-to solution for the current corporate sector worldwide, in the event of a cyber-attack. 
%
However, even as cyber-insurance contracts with premiums worth billions of dollars are underwritten annually, one of the prevailing concerns among insurers is the quantitative understanding of major/catastrophic risks and how risks accumulate and aggregate, as cyber-risks spread via network connectivity and vendor relationships. 
%However, market surveys suggest that demand for cyber-insurance significantly exceeds the capacity currently provided by the insurance industry. The primary reason that most insurers give for being cautious about expanding capacity is the accumulation risk posed by cyber-threats. The main fear among insurers here is that cyber-threats are inherently scalable and systemic through their spread via network interconnectivity -  
For instance, a single malicious email generated by a botnet activity as part of a social engineering attack can paralyze an entire firm and completely disrupt its services; this in turn can disrupt the services provided by its customers, and that provided by its customers' customers.  As the multitude of losses are attributed to the original firm, who carries third-party liability insurance, its policy is potentially faced with 
%In the event of cascading service disruptions due to a major cyber-attack, if all these organizations were to hold responsible their parent organization(s) on which they depend on for providing services, it is quite likely that the insurance company of a certain root organization could need to bear the responsibility of covering a 
huge aggregate risks accumulated over the supply chain \cite{millaire}. This motivates insurers to seek reinsurance, as they do in more traditional areas, but a critical differentiation here is that a cyber-reinsurer is more or less faced with the same risk aggregation and accumulation issue because the traditional method of spreading risk (over different industry sectors, geographic locations, firm sizes, and so on) has only limited effect in the cyber domain due to the risk correlation induced by connectivity and supply chain relationship described above. 
%Shouldering this responsibility clearly may not be aligned with satisfying the budget constraints and profit requirements of most risk-averse cyber-insurers open to the idea of providing re-insurance services, leave alone cyber-forensic and risk data availability challenges they might need to overcome to implement accumulative coverage policies \cite{millaire}. 
Toward this end, this letter sets out to analyze what happens when i.i.d. cyber-risks of a heavy-tailed nature are aggregated, and whether traditional risk spreading is reliable, and under what conditions. Here, the term `reliability' is synonymous with the aggregate cyber-risk distribution not increasing in spread with the number of cyber-risks aggregated. Our analysis further allows us to envision whether providing cumulative risk services such as reinsurance is statistically incentive compatible for the reinsurer post catastrophic cyber-attack events.
% \textbf{Our Focus -} Our focus in this paper is to analyze conservatively whether providing accumulative risk services (e.g., re-insurance) is statistically incentive compatible for the cyber-insurance industry. Our investigation is of immense importance to societal benefit in the age where IT-networked services are ubiquitous in nature and complex cyber-attacks, both on commercial and critical infrastructures, are on the rise. 
This is of immense importance as failure to effectively manage cyber-risk via reinsurance could negatively impact the ability of front-line insurers to offer loss coverage via a sustainable market mechanism, and contribute to a depressed society. 
% or a lack of proper aggregate risk covering markets could really mean bad for societal welfare in general as cyber-insurance companies could individually opt out of covering aggregated cyber-risk, and a spiral effect could lead to the break-down of a significant portion (if not entirely) of the much needed and existing traditional cyber-insurance industry. 
This could also negatively impact overall cyber-security, which is theorized in literature (see \cite{hoffman}\cite{lelarge2009economic}\cite{ssfw}\cite{pal2011aegis}\cite{pal2014will}\cite{rpinfr2018}\cite{khalili2018designing}\cite{naghizadeh2014voluntary}\cite{rabohme}) to improve with a successful, expanding, and maintainable cyber-insurance markets. %; the reader is referred to Section \ref{related} for literature on how cyber-insurance can help improve network security. 
%in the network of organizations tied to one another via commercial liability relationships. On the contrary, the realistic possibility of the existence of successful aggregate cyber-risk coverage markets opens up the scope of further investigation into (a) cost aspects of acquiring cyber-risk information and data to make these markets working to scale, and (b) the likelihood, i.e., probability as a function of the business liability network parameters, of extreme events that might put coverage pressure on working aggregate cyber-risk coverage markets. 
%\subsection{Research Contributions}

More specifically, as main contributions in this letter, we first use standard methods to study the impact of (catastrophic) cyber-risk distributions being heavy-tailed. Using typical examples of such distributions (with infinite statistical moments such as mean and variance), we show in Section III via the popular Value-at-Risk (VaR) risk measure that aggregating such i.i.d. cyber-risks can result in a risk distribution whose spread (i.e., variance) increases with the number of statistically independent cyber-risks aggregated. %This is most likely to have a dampening effect on the feasibility mindset of cyber-risk managers to provide coverage for aggregated cyber-risks. 
This unreliability of the cyber-risk spreading with respect to aggregate cyber-risk management directly impacts the statistical incentive compatibility of the risk aggregation business and thus the feasibility of reinsurance as a business model. For this reason, this increase in risk spread will also be referred to as the {\em infeasibility of catastrophic risk aggregation in this letter.} 
%We prove that this result also extends to the case of aggregating independent but non-identical catastrophic cyber-risks (Section \ref{sec:analysis})
We further show in Section \ref{sec:curtail} the somewhat surprising result that the aforementioned worsening of risk spread also holds in \emph{many} %(a function of the number of cyber-risks to be aggregated, the extent of curtailment, and cyber-risk valuation) 
cases (and consequently derive precise mathematical `holding' conditions) when these heavy-tailed distributions are curtailed in their statistical support so that they now have finite support and finite statistical moments; this is equivalent to policies imposing coverage limits on claimable losses.
%More precisely, we derive mathematical conditions under which the worsening of aggregate cyber-risk spread holds, and vice versa. 
%
%The results demonstrate that the issue of worsening risk spread does not \emph{solely} arise from the extreme tails of risk distributions, as one may intuitively think; the nature of the aggregator's utility function and the number of cyber-risks to be aggregated also play a significant role to play.
%To this end, we also show that risk aggregation is increasingly infeasible for bounded heavy-tailed cyber-risks when the aggregator's utility function at any point in the domain of large negative outcomes becomes convex.

 %\ref{sec:curtail}).
%\end{itemize}

%To the best of our knowledge, the above represents the first general (and considerably complete) mathematical characterization on the feasibility of covering aggregate (independent and dependent) catastrophic cyber-risks.  
%In essence, our results suggests that in events of catastrophic cyber losses with unbounded statistical support, imposing coverage limits alone might not be sufficient 
%\emph{always} provide much positive boost to the 
%for for-profit risk aggregators such as reinsurers. 
%Ultimately, in such situations government agencies might be the best sources to resort to for managing aggregate cyber-risks, in addition to relying on for-profit industries. At the same time, our results also highlight the criticality of risk control in the first place given potentially limited ability to transfer.

%\rev{The remainder of the paper is organized as follows. XXXXX} 


